S1-NexusAgent: a Self-Evolving Agent Framework for Multidisciplinary Scientific Research

Modern scientific research relies on large-scale data, complex workflows, and specialized tools, which existing LLMs and tool-based agents struggle to handle due to limitations in long-horizon planning, robust goal maintenance, and continual learning from execution. To address these issues, in this work, we propose S1-NexusAgent, a self-evolving agent framework designed for multidisciplinary scientific research. S1-NexusAgent adopts a hierarchical Plan-and-CodeAct execution paradigm, decoupling global scientific planning from subtask-level tool execution through a dual-loop architecture, thereby enabling stable modeling of complex research workflows. The system natively supports the Model Context Protocol (MCP), integrates up to thousands of cross-disciplinary scientific tools, and achieves efficient orchestration of heterogeneous research tools via intention-aware dynamic tool retrieval and hot-plug mechanisms. To address long-context and large-scale data challenges in scientific settings, S1-NexusAgent introduces object-reference-based sparse context management, which enables sub-task context isolation and intermediate result compression. Building on this, a Critic Agent automatically evaluates complete execution trajectories and distills high-quality research paths into reusable Scientific Skills, forming a closed loop for continuous self-evolution, which is valuable for sustainable and long-horizon scientific research. Experiments on authoritative scientific benchmarks involving long-horizon planning and complex specialized tool orchestration, including biomini-eval (biology), ChemBench (chemistry), and MatSciBench (material science), demonstrate that S1-NexusAgent achieves state-of-the-art performance, validating its effectiveness and generalization capability in complex scientific tasks.

==> 3_architecture_sections/4_CodeAct_and_MCP.tex <==
% \subsection{An Extensible Scientific Tool Ecosystem}
% \label{sec:codeact_mcp}
% During the subtask execution stage, S1-NexusAgent adopts CodeAct as a unified action interface, enabling the agent to interact with real scientific tools through executable reasoning. Within CodeAct, a Code Agent synchronously produces two complementary components for each assigned subtask: (1) an explicit reasoning trace that articulates the underlying scientific hypotheses, tool-selection rationale, and execution strategy; and (2) executable code that can be directly run in a sandboxed environment to drive concrete scientific computations, data analyses, or simulation tasks. All generated code is executed within an isolated Sandbox Environment, ensuring execution safety and reproducibility.

% % --- Figure 5: Tool Ecosystem ---
% \begin{figure*}[!htp]
%     \centering
%     \includegraphics[width=0.85\textwidth]{figures/tool_ecosystem.png}
%     \caption{\textbf{The modular and extensible scientific tool ecosystem of S1-NexusAgent.} Scientific capabilities are abstracted into three functional layers: domain-specific tools (e.g., bioinformatics, materials simulation), literature retrieval services, and general utilities. By adopting CodeAct as the unified action paradigm and maintaining compatibility with standardized tool protocols, S1-NexusAgent provides a secure, sandboxed environment for programmatic tool interaction, enabling seamless integration of diverse scientific instruments and databases without model retraining.}
%     \label{fig:tool_ecosystem}
% \end{figure*}

% S1-NexusAgent natively supports the Model Context Protocol (MCP), which abstracts scientific tools from diverse sources into standardized interfaces. The resulting tool ecosystem spans a wide range of scientific use cases and can be broadly categorized into three classes according to functionality as follows.

% \paragraph{(1) Domain-Specific Scientific Tools.}These tools target specific scientific domains and provide highly specialized computational and analytical capabilities, including but not limited to life sciences, chemistry, materials science, and astronomy. This category also includes general-purpose scientific computing and mathematical tools for numerical computation, statistical analysis, and model solving. Together, these tools form the core capability foundation for professional scientific reasoning and experimental simulation.

% \paragraph{(2) Literature and Information Retrieval Tools.}This class of tools is designed to acquire and integrate external scientific knowledge, such as academic literature search engines, domain-specific database interfaces, and cross-source information aggregation services. By enabling dynamic access to up-to-date and relevant background knowledge during task execution, these tools prevent isolated reasoning and enhance scientific rigor.

% \paragraph{(3) General Utility Tools.}Utility tools provide common auxiliary functions required in scientific workflows, including web content crawling and parsing, file format conversion, and URL-based file packaging. While these tools do not directly perform scientific modeling, they play a critical supporting role in constructing end-to-end research pipelines, automating data preparation, and organizing experimental outputs.

% Through standardized tool interfaces, tool functionality descriptions, input–output schemas, and execution constraints can be automatically interpreted and invoked by the agent. This design enables continuous expansion of the tool ecosystem without requiring retraining of the core models, thereby supporting long-term scalability and extensibility of the system.

